Safe-DS: A Domain Specific Language to Make Data Science Safe

Due to the long runtime of Data Science (DS) pipelines, even small programming mistakes can be very costly, if they are not detected statically. However, even basic static type checking of DS pipelines is difficult because most are written in Python. Static typing is available in Python only via external linters. These require static type annotations for parameters or results of functions, which many DS libraries do not provide. In this paper, we show how the wealth of Python DS libraries can be used in a statically safe way via Safe-DS, a domain specific language (DSL) for DS. Safe-DS catches conventional type errors plus errors related to range restrictions, data manipulation, and call order of functions, going well beyond the abilities of current Python linters. Python libraries are integrated into Safe-DS via a stub language for specifying the interface of its declarations, and an API-Editor that is able to extract type information from the code and documentation of Python libraries, and automatically generate suitable stubs. Moreover, Safe-DS complements textual DS pipelines with a graphical representation that eases safe development by preventing syntax errors. The seamless synchronization of textual and graphic view lets developers always choose the one best suited for their skills and current task. We think that Safe-DS can make DS development easier, faster, and more reliable, significantly reducing development costs.

==> backup-rolesInDS.tex <==
% \section{Roles in DS}
% \label{sec:roles-in-ds}


% \discussion{Vorschlag:}

% In order to design languages and tools that help the people involved in the development of data science applications, we first need to know who these people are.  
% %We first need to understand the people involved in DS. 
% Based on \cite{maoHowDataScientists2019, mullerHowDataScience2019, zhangHowDataScience2020} and the 2021 Kaggle DS survey \cite{kaggle2021KaggleMachine}, we derived the following roles that are relevant in our context:

% \paragraph*{DS Students} We refer to people who want to learn about DS as \keyword{DS Students}, regardless of whether they are enrolled in a university, participate in an online course, or use other learning resources. DS Students typically have some programming skills but little to no DS experience. 
% %According to a survey by ... (<-- aus dem Vortrag von eben) more than 60\% of data scientists have no programming background. 
% Their primary goal is learning to use concepts and APIs, rather than solving a specific business problem satisfactorily. 
% %Often, business problems published by others, e.g. via Kaggle\footnote{\url{https://kaggle.com}}, are used as exercises. 

% Applying DS methods to solve business problems is the focus of two other roles: 
% \begin{itemize}
%     \item \keyword{Domain Experts}, who know the problem domain but usually have neither programming nor DS skills.
%     \item \keyword{Data Scientists}\footnote{We do not differentiate this role further since it is irrelevant for the following discussion.}, who develop the DS pipeline that eventually creates insight about the data. They typically have good programming and DS skills but rely on the Domain Experts for domain knowledge. Moreover, they have an established toolkit of techniques, languages, libraries, and other tools to create a DS pipeline regardless of the business problem.
%     %\item \keyword{End Users}, who use the solution developed by the Domain Experts and Data Scientists for the business problem. They are often not interested in how the solution was obtained and are neither required to have programming nor DS expertise. Some domain knowledge can be expected, however.
% \end{itemize}

% \paragraph*{DS Researchers} Finally, \keyword{DS Researchers} enhance existing DS methods, or create entirely new ones. Their research can be focused on a specific business problem but is often applicable in a larger context. The result of their work % can either way be 
% is typically made available to Data Scientists
% via contribution to various DS libraries. DS Researchers need excellent understanding of DS and strong programming skills to 
% %prototype their ideas. 
% achieve efficient implementations of their ideas. 
% %
% Like Data Scientists, they already have a set of tools to implement their contributions. %these prototypes.

% %In the following, we refer to students and domain experts together as \keyword{DS novices}, and to data scientists and researchers as \keyword{DS experts}. 

% We want to highlight some observations about the above roles:
% %
% \begin{itemize}
%     \item DS Researchers need highly expressive tools to be able to \emph{extend} the DS landscape. 
%     Using the same tools can be overwhelming and useless for the other three roles, which just need to \emph{reuse} existing APIs and \emph{configure} them for their current use case. In the following we focus on the needs of students, domain experts and DS experts. Together, we call them our traget users.
    
%     \item Different roles have \emph{vastly different skill levels} regarding programming and DS. The lower the skills, the greater the need for guidance \cite{reimannAchievingGuidanceApplied2020a} when developing a DS pipeline to ensure correctness and adherence to DS best practices. 
%     %
%     \todo{Derive safety and flexibility requirements from the guidance idea.}
    
%     \item Due to 
%     % the lack of domain knowledge and DS knowledge respectively, 
%     their complementary skills,
%     \emph{Data Scientists and Domain Experts must collaborate with each other} \cite{maoHowDataScientists2019, zhangHowDataScience2020}. 
%     For this collaboration, a common understanding of the problem, and the ability to verify a solution are crucial. 
%     This is difficult, however, because of the 
%     % difference in skills and the resulting <-- weglassen, da schon fünf Zeilen weiter oben gesagt?
%     lack of a common language.
% \end{itemize}
% ====================================================================



% --------------------

% \discussionbefore{Bisher:}
% We want to highlight some observations about the list of roles from Sec. \ref{sec:roles-in-ds}:
% %
% \begin{itemize}
%     \item DS Researchers \emph{extend} the DS landscape, while the others \emph{reuse} methods that are already available and \emph{configure} them for their current use case. While DS Researchers need highly expressive tools for their task, building blocks developed by them can be reused using simpler systems.
%     \item Different people have \emph{vastly different knowledge levels} regarding programming and DS. The lower the knowledge level, the greater the need for guidance \cite{reimannAchievingGuidanceApplied2020a} when developing a DS pipeline to ensure correctness and adherence to DS best practices. \discussionafter{Talk about safety instead? It's in the name of the DSL and allows a more targeted RQ 3 (different views are also a means to provide guidance). Downside: Harder to cite first paper :)}
%     \item Due to the lack of domain knowledge and DS knowledge respectively, \emph{Data Scientists must collaborate with Domain Experts} \cite{maoHowDataScientists2019, zhangHowDataScience2020}. For this collaboration, a common understanding of the problem and the ability to verify a solution are crucial. This is difficult, however, because of the difference in skills and the resulting lack of a common language.
% \end{itemize}

% %\paragraph*{DS Education} The goal of DS Education is to teach existing DS methods, rather than solving a specific business problem satisfactorily. 
% %% Published business problems, e.g. from Kaggle\footnote{\url{https://kaggle.com}}, can be used as exercises. 
% %We refer to people who want to learn about DS as \keyword{DS Students}, regardless of whether they are enrolled in a university, participate in an online course, or use other learning resources. DS Students typically have some programming skills but little to no DS experience. 
% %%

% %\paragraph*{Applied DS} The objective of Applied DS is to apply existing DS methods to solve a specific business problem. We assume that enough data is already available. This process involves two distinct roles: 
% %%
% %\begin{itemize}
% %    \item \keyword{Domain Experts}, who know the problem domain but usually have neither programming nor DS skills.
% %    \item \keyword{Data Scientists}\footnote{We do not differentiate this role further since it is irrelevant for the following discussion.}, who develop the DS pipeline that eventually creates insight about the data. They typically have good programming and, naturally, DS skills but rely on the Domain Experts for domain knowledge. Moreover, they have an established toolkit of techniques, languages, libraries, and other tools to create a DS pipeline regardless of the business problem.
%     %\item \keyword{End Users}, who use the solution developed by the Domain Experts and Data Scientists for the business problem. They are often not interested in how the solution was obtained and are neither required to have programming nor DS expertise. Some domain knowledge can be expected, however.
% %\end{itemize}

% %\paragraph*{DS Research} Finally, \keyword{DS Researchers} enhance existing DS methods or create entirely new ones. Their research can be focused on a specific business problem but is often applicable in a larger context. The result of their work can either way be made available to Data Scientists. We expect them to have an excellent understanding of DS and sufficient programming skills to prototype their ideas. Like Data Scientists they already have a set of tools to implement these prototypes.

% \todo{
% \begin{itemize}
%     \item Integrate different roles into introduction
%     \item Motivate before state of the art that guidance is needed
%     \item Safety is a part of guidance. The latter can also include tutorials, pair programming with an experienced Data Scientist, etc.
%     \item Different views and static checking both offer safety
%     \item Add some criticism to the state of the art (e.g. Ludwig's configuration offers no safety, only runtime errors)
%     \item Motivate lack of loops and conditionals: No need for them since pipelines are sequential. Loops/decisions are either inside of building blocks or external to the system, in the user's workflow (Which model should I choose? pick one, use it, evaluate, repeat)
% \end{itemize}
% }

==> backup-xyz.tex <==


% \todo{
%     \begin{itemize}
%         \item RQ 1
%         \item --- pipelines
%         \item No need to model all things data science in the language itself. We instead have more generic concepts like functions in there.
%         \item Language concepts:
%         \item Data: Literals (constant values), placeholders (names for, potentially computed, values)
%         \item Literals: Boolean, Number, String, null
%         \item Placeholder: Can be referenced by name in other places of the program
%         \item Assignment: Set value of a placeholder - can only be assigned once / cannot be reassigned (name for one fixed value)
%         \item Process: One step in a pipeline (can be external in python or implemented in the language itself)
%         \item Call: Trigger execution of a process; pass inputs (parameters); get back outputs (results)
%         \item No loops, conditionals. Can instead use more concrete concepts like hyper parameter optimization, which hide loops and conditionals internally. Can treat these as blackboxes.
%         \item No loop, conditionals. These exist in the user development pipeline (choose model, validate, choose another model or tweak it, validate again...) but are rarely needed in the code itself since higher abstractions can be offered (hyperparameter optimization, training functions etc.)
%         \item Example for development flow: CRISP DM
%         \item --- Stubs
%         \item Stub language needed to glue the \safeds{} world and the Python world together
%         \item ---
%         \item Different sublanguages: Stub language, pipeline language
%         \item Immutability; placeholders cannot be reassigned (shallow immutability); deep immutabilty requires proper implementation in the adapters; could also implement deep immutability in compiler (generate copy operations on demand, only if later mutation is used)
%         \item Purity (caching + partial evaluation) / no side effects (partial evaluation) --- appropriate annotations; also parellelization
%         \item Explicit annotations / types / metainformation in stub language
%         \item Inference in pipeline language, where possible. Only write types of pipeline steps explicitly for reuse. Otherwise, we'd not be able to implement recursion. Can later be relaxed for places that don't use recursion. Can also just dump everything into the main pipeline, so the user does not need to worry about types. Downside: No reusability but can later be refactored (e.g. by someone else). Initially getting a model for a single use case is the most important thing for our main target users (e.g. domain experts)
%         \item Maybe also introduce pipeline steps only as a means to achieve reusability in the DSL and start just with the pipeline.
%         \item Type parameters needed for generic transformations
%         \item Parameters can be optional (with a default value) or required
%         \item Sometimes the behavior of a process must be adjusted at a specific point (e.g. when transforming a column of a tabular dataset)
%         \item Solution: Higher-order functions, lambdas for ease of use (type inferred from schema information and stubs). Need to come up with less "frightening" name (e.g. configurable processes? Though any process with inputs is configurable)
%         \item Based on dataflow compiler can implicitly parallelize (petri nets)
%         \item Partial evaluation (for static checking and optimization)
%         \item "Baukastenprinzip" --- no loops, ability to integrate external processes into \safeds{}; language can be simple and easy to analyze; still extensible; hides complexity from \safeds{} user
%         \item Stub language necessarily influenced by Python (since we want to make Python libraries available); however, we omitted some things like overloaded operators since we believe named program elements are better for usability)
%         \item Key elements of stub language:
%         \item Class
%         \item Enum
%         \item Function + Parameters/Results
%         \item Annotations (additional metainformation, e.g. purity, documentation etc.)
%         \item Standard library also uses stubs; shipped with language, no need to reinvent the wheel for each pipeline; makes several libraries available (WIP)
%         \item Stubs must correspond to Python implementation
%     \end{itemize}
% }
